Analysis of Quantum Entanglement in Quantum Programs using Stabilizer Formalism

Quantum entanglement plays an important role in quantum computation and communication. It is necessary for many protocols and computations, but causes unexpected disturbance of computational states. Hence, static analysis of quantum entanglement in quantum programs is necessary. Several papers studied the problem. They decided qubits were entangled if multiple qubits unitary gates are applied to them, and some refined this reasoning using information about the state of each separated qubit. However, they do not care about the fact that unitary gate undoes entanglement and that measurement may separate multiple qubits. In this paper, we extend prior work using stabilizer formalism. It refines reasoning about separability of quantum variables in quantum programs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{262}
\providecommand{\publicationstatus}{Chris Heunen, Peter Selinger, and Jamie Vicary (Eds.):\\
12th International Workshop on Quantum Physics and Logic (QPL 2015).\\
EPTCS 195, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.195.19}{10.4204/EPTCS.195.19}}
\pdfoutput=1

